VR-Goggles for Robots: Real-to-sim Domain Adaptation for Visual Control

In this paper, we deal with the reality gap from a novel perspective, targeting transferring Deep Reinforcement Learning (DRL) policies learned in simulated environments to the real-world domain for visual control tasks. Instead of adopting the common solutions to the problem by increasing the visual fidelity of synthetic images output from simulators during the training phase, we seek to tackle the problem by translating the real-world image streams back to the synthetic domain during the deployment phase, to make the robot feel at home. We propose this as a lightweight, flexible, and efficient solution for visual control, as 1) no extra transfer steps are required during the expensive training of DRL agents in simulation; 2) the trained DRL agents will not be constrained to being deployable in only one specific real-world environment; 3) the policy training and the transfer operations are decoupled, and can be conducted in parallel. Besides this, we propose a simple yet effective shift loss that is agnostic to the downstream task, to constrain the consistency between subsequent frames which is important for consistent policy outputs. We validate the shift loss for artistic style transfer for videos and domain adaptation, and validate our visual control approach in indoor and outdoor robotics experiments.

==> secs/experiments-adaptation-comparison.tex <==
\subsection{Comparing Domain Adaptation Methods: Real-world Indoor \& Outdoor Navigation}
\label{sec:experiments-adaptation-comparison}


\begin{figure*}[!t]
    \includegraphics[width=\textwidth]{imgs/realworld}
    \label{fig:realworld}
  \vspace{-0.25in}
  \caption{
Real-world visual control experiments.
\textit{\textbf{Indoor}} (yellow):.
A navigation policy (\textit{From-Scratch}, Sec. \ref{sec:experiments-transfer-comparison})
is firstly trained in a simulated environment
(\textit{Sim-Env}, Fig. \ref{fig:transfer-compare})
that is able to navigate to chairs based on visual inputs.
Without retraining or finetuning,
our proposed \textit{VR-Goggles} enables the mobile robot to
directly deploy this policy in an office environment,
achieving $100\%$ success rate in a set of real-world experiments.
Here \textit{Miss} refers to test runs
\hl{where the agent does not know what to do due to the \textit{reality gap}
or due to the unsatisfied quality of the translated image,}
or when it simply ignores the chair even when they are in sight;
\textit{Hit} refers to frames where the agent captures the chair in sight
and outputs commands to move towards it.
\textit{\textbf{Outdoor}} (cyan):
An autonomous driving policy (via conditional imitation learning \cite{Codevilla2018})
is trained in \textit{Carla} daytime,
a \textit{VR-Goggles} model is trained to translate
between \textit{Carla} daytime and \textit{Robotcar} nighttime,
which enables the real-world nighttime deployment of the trained policy.
More details are presented in the attached video.
  % A DRL agent is trained in a simulated office environment, that is able to navigate to chairs based on visual input.
  % Without retraining or finetuning the DRL policy, our proposed \textit{VR-Goggles} enables the mobile robot to directly deploy this policy in real office environments, achieving $100\%$ success rate in a set of real-world experiments. We refer to the attached video for details of the real-world experiments.
  }
  \label{fig:realworld}
\end{figure*}

We conduct real-world robotics experiments for both indoor and outdoor visual navigation tasks.
We begin by training learning-based visual navigation policies,
taking simulated first-person-view images as inputs,
outputting moving commands for specific navigation targets.
Then, we deploy the trained policy onto real robots,
% in real-world environments,
comparing the following \textit{domain adaptation} approaches:
(1) \textit{\textbf{No-Goggles}}: Feed the sensor readings directly to the DRL policy;
(2) \textit{\textbf{CycleGAN}}/\textit{\textbf{CyCADA}} \cite{zhu2017unpaired,hoffman2017cycada}: Use \textit{CycleGAN} (when semantic ground truth is not available) / \textit{CyCADA} (when ground truth semantic maps are provided by the simulator) to translate the real sensory inputs to the synthetic domain before feeding
to policy nets;
(3) \textit{\textbf{Ours}}:
Add \textit{shift loss} on top of (2)
% Use models trained by \textit{CycleGAN}/\textit{CyCADA} $+$ \textit{shift loss}
as the \textit{\textbf{VR-Goggles}}.
% to translate the input images.

% We validate our proposed method of using the \textit{\textbf{VR-Goggles}} to facilitate the transfer of polices trained in the simulated domain to the realistic domain, with a set of real-world robotic experiments.

\input{secs/experiments-indoor-control}
\input{secs/experiments-outdoor-control}


==> secs/experiments-carla-transfer.tex <==
% \subsection{\textit{Domain Adaptation} for \textit{Outdoor} Scenarios}
\subsection{Comparing Domain Adaptation Methods: Outdoor Navigation}
\label{sec:experiments-carla-transfer}

\hl{Since there is no commonly used benchmark for real-world navigation evaluation,}
We first test our \textit{domain adaptation} method in \textit{Carla} simulator following the benchmark setup in \cite{dosovitskiy2017carla} and the imitation learning method in \cite{dosovitskiy2017carla, Codevilla2018}.
We deploy the trained policy to a previously unseen weather condition through three different domain adaptation approaches:
(1) \textit{\textbf{No-Goggles}}: Feed the sensor readings directly to the policy;
(2) \textit{\textbf{CycleGAN}} \cite{zhu2017unpaired}: Use \textit{CycleGAN} to translate the real sensory inputs to the synthetic domain before feeding
to policy nets;
(3) \textit{\textbf{Ours}}:
Add \textit{shift loss} on top of (2) as the \textit{\textbf{VR-Goggles}}.

In \cite{dosovitskiy2017carla}, the expert datasets are collected under $4$ different weather conditions (\textit{daytime}, \textit{daytime after rain}, \textit{daytime hard rain} and \textit{clear sunset}). The trained policy was tested in benchmark tasks under \textit{cloudy daytime} and \textit{soft rain at sunset}. Since the datasets of their testing benchmark conditions are not available\footnote{https://github.com/carla-simulator/imitation-learning} for us to conduct domain adaptation, we split the provided training datasets to training conditions (\textit{daytime}, \textit{daytime after rain}, \textit{clear sunset}) and testing condition (\textit{daytime hard rain}).

For each of the $3$ training conditions, we train a \textit{Single-Domain} policy. We also train a \textit{Multi-Domain} policy with all $3$ training whether conditions.
%We follow the branched structure in \cite{Codevilla2018} to train the related navigation policy.
% The \textit{Mult-Domain} policy can be regared as a navive domain randomization method.

For adapting the trained policy to the testing weather condition, for both the \textit{CycleGAN} and the \textit{VR-Goggles} strategy, we train an adaptation network \hl{from} the testing condition \hl{to} each of the $3$ training conditions.
(For more details about the training of the policy and adaptation models please refer to \hl{the suplmentatry file in web} \footnote{https://ram-lab.com/file/tailei/vr\_goggles/index.html}.)

Table \ref{tab:carla_metric} shows the benchmark evaluation results,
all of the metrics are the standard output from the released code\footnote{https://github.com/carla-simulator/carla/tree/0.8.2} as in \cite{dosovitskiy2017carla}.
The results for 3 \textit{Single-Domain} policies are averaged in the table. For the \textit{Multi-Domain} policy, we evaluat it for each of the $3$ training conditions and show the averaged results.
The evaluation of our trained policies under the training conditions show comparable results as the original result in \cite{dosovitskiy2017carla}.
% For training conditions, the single condition result is the averaged result across all the three single condition polices under their own training weathers individually.
% The domain random result is the averaged result across all of its three training weathers.
For the testing under the new weather condition, all policies are evaluated under the \textit{daytime hard rain} weather in the benchmark.
For each of the \textit{single-domain} policy, the visual inputs are translated by the adaptation model from \textit{daytime hard rain} to the corresponding training weather condition.
We average the results of the $3$ \textit{Single-Domain} polices as well.
\hl{is this description correct?:} For the \textit{Multi-Domain} policy, we evaluate it three times for all transfer strategies through each of the transfer model to transfer the input image under hard rain to one of its training condition.
We average the results of \textit{Multi-Domain} policy under the $3$ transfer models as well.

The four benchmark tasks (\textit{Straight}, \textit{One Ture}, \textit{Navigation}, \textit{Nav. dynamic}) are in order of increasing difficulties \hl{where each of them consists of 25 different defined travelling episodes}.
Unlike the original setup in \cite{dosovitskiy2017carla}, directly deploying the policy in the testing weather can finish none of the two harder tasks, which could be explained by our using fewer domains (weather conditions) of data to train the policy and deploying it in a more extreme weather condition. For the different transfer strategies, our \textit{VR-Goggles} outperforms \textit{CycleGan} in almost all of the metrics, especially the two harder tasks (\textit{Navigation} and \textit{Navigation with dynamic obstacles}) in both the success rate and the average percentage of distance to goal traveled.
The average distance traveled between two infractions in is reported as in \cite{dosovitskiy2017carla} for the hardest task, which is navigating in the presence of dynamic objects.
The adaptation models of \textit{Ours} enable the agents to run safely with lower frequencies (\hl{what is frequencies}) or comparable frequencies (0.05 lower in opposite lane for single-domain policies) \hl{for suffering most of the infractions compared with \textit{CycleGAN}}.
\textit{CycleGAN} collides with pedestrains less often with the \textit{Multi-Domain} policy.
A probable explanation is that most of episodes under this setup end due to collision with cars and static obstacles.
It does not suffer too many challenging pedestrian conditions.
For example, for direct deploy without adaptation, the avergate distance between collision with pedestrains is higher than 4.6 km, becasue the total navigation distance for all the episodes in this task is only 4.6 km and it is too short to encounter pedestrians.

Notice that the transfer pipelines of the \textit{Single-Domain} policy are behaving much better than directly deploying the \textit{Multi-Domain} policy; moreover, the training time of the former policy is also much shorter than the latter one.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
% \begin{tabular}{llcclccclccc}
\begin{tabular}{llcclccclccc}
\hline
                                                                                                                      &                      & \multicolumn{2}{c}{Training }                                                                                                                           &  & \multicolumn{7}{c}{New weather}                                                                  \\ \cline{3-12}
                                                                                                                      &                      & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Single-\\ Domain\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Multi-\\ Domain\end{tabular}} &  & \multicolumn{3}{c}{Single-Domain} &  & \multicolumn{3}{c}{Multi-Domain}                  \\
                                                                                                                      &                      &                                                                             &                                                                          &  & No-Goggles  & CycleGAN         & VR-Goggles          &  & No-Goggles                & CycleGAN         & VR-Goggles          \\ \hline
\multirow{4}{*}{Success rate (\%)}                                                                                    & Straight             & 81.3                                                                        & 97.3                                                                     &  & 13.3 & \textbf{93.3} & 90.7          &  & 64.0               & 96.0          & \textbf{100}  \\
                                                                                                                      & One turn             & 64.0                                                                        & 85.3                                                                     &  & 1.3  & \textbf{54.7} & \textbf{54.7} &  & 36.0               & 61.3          & \textbf{76.0} \\
                                                                                                                      & Navigation           & 60.0                                                                        & 84.0                                                                     &  & 0.0  & 21.3          & \textbf{45.3} &  & 0.0                & 42.7          & \textbf{61.3} \\
                                                                                                                      & Nav. dynamic         & 58.7                                                                        & 74.7                                                                     &  & 0.0  & 21.3          & \textbf{32.0} &  & 0.0                & 34.7          & \textbf{56.0} \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Average percentage \\ of distance to \\ goal traveled (\%)\end{tabular}}   & Straight             & 89.7                                                                        & 96.5                                                                     &  & 37.8 & \textbf{95.8} & 94.7          &  & 83.6               & 95.9          & \textbf{98.3} \\
                                                                                                                      & One turn             & 73.6                                                                        & 71.1                                                                     &  & 18.4 & 36.3          & \textbf{48.4} &  & 24.7               & 52.0          & \textbf{71.3} \\
                                                                                                                      & Navigation           & 68.6                                                                        & 88.8                                                                     &  & 7.3  & 36.7          & \textbf{51.0} &  & 7.4                & 60.8          & \textbf{73.1} \\
                                                                                                                      & Nav. dynamic         & 68.2                                                                        & 80.7                                                                     &  & 5.0  & 32.6          & \textbf{51.3} &  & 5.2                & 55.7          & \textbf{72.2} \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}Average distance \\ traveled between \\ two infractions in \\ Nav. dynamic (km)\end{tabular}} & Opposite lane        & 2.83                                                                        & 2.55                                                                     &  & 0.23 & \textbf{0.77} & 0.72          &  & 0.26               & 0.83          & \textbf{2.22} \\
                                                                                                                      & Sidewalk             & 6.47                                                                        & 9.70                                                                     &  & 0.21 & 1.15          & \textbf{2.62} &  & 0.38               & 1.29          & \textbf{2.46} \\
                                                                                                                      & Collision-static     & 2.38                                                                        & 3.03                                                                     &  & 0.14 & 0.52          & \textbf{0.87} &  & 0.16               & 0.77          & \textbf{1.26} \\
                                                                                                                      & Collision-car        & 2.06                                                                        & 1.03                                                                     &  & 0.29 & 1.01          & \textbf{1.40} &  & 0.27               & 0.59          & \textbf{0.77} \\
                                                                                                                      & Collision-pedestrian & 15.10                                                                       & 16.17                                                                    &  & 2.17 & 4.03          & \textbf{6.98} &  & \textgreater{}4.60 & \textbf{7.29} & 4.67          \\ \hline
\end{tabular}
\caption{Quantitative evaluation of go-directed navigation tasks following \cite{dosovitskiy2017carla}. We train control policy through imitation learning from single weather condition (\textit{Single-Domain}) and multiple weather conditions (\textit{Multi-Domain}). Policies are tested in new weather conditions through direct deploying (Raw), transfering the input image through \textit{CycleGAN} (CyG) and transfering through \textit{Ours} with \textit{shift loss}. Higher is better.}
\label{tab:carla_metric}
\end{table*}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{imgs/carla_weathers/daytime}
    \includegraphics[width=0.45\textwidth]{imgs/carla_weathers/wet}
    \includegraphics[width=0.45\textwidth]{imgs/carla_weathers/sunset}
    \includegraphics[width=0.45\textwidth]{imgs/carla_weathers/rain}
    \caption{carla weather}
    \label{fig:carla_conditions}
\end{figure}


==> secs/experiments-outdoor-domain-adaptation.tex <==
\subsection{\textit{Domain Adaptation} for \textit{Outdoor} Scenarios}
\label{sec:experiments-outdoor}


\begin{figure}[!b]
    \centering
        \includegraphics[width=0.45\textwidth]{imgs/domain_adapt/carla2robotcar}
    \vspace{-0.01in}
    \caption{
    Comparison of the translated images for sequential input frames for the different approaches.
    $\nth{1}$ \textit{row}: two subsequent input frames from the realistic domain, with several representative images from the simulated domain shown in between;
    $\nth{2}\sim\nth{4}$ \textit{row}: outputs from \textit{CyCADA}, \textit{CyCADA+flow} and \textit{Ours}.
    Our method is able to output consistent subsequent frames and eliminate artifacts.
    We adjust the brightness of some zoom-ins for visualization purposes.}
    \label{fig:carla2robotcar}
\end{figure}

Next we validate the \textit{shift loss} in the field of \textit{domain adaptation}, firstly in \textit{outdoor} urban street scenarios (where we collect synthetic domain images $\bX\sim p_{\text{sim}}$ from the \textit{CARLA} simulator \cite{dosovitskiy2017carla}, and realistic domain images $\bY\sim p_{\text{real}}$ from the \textit{RobotCar} dataset \cite{RobotCarDatasetIJRR}). We compare the following three setups:
% \begin{itemize}
(1)\textit{CyCADA} \cite{hoffman2017cycada}: \textit{CycleGAN} with semantic constraints, trained on single frames;
(2)\textit{CyCADA+flow}: \textit{CyCADA} with temporal constraints (\cite{huang2017real}), trained on sequential frames;
(3)\textit{Ours}: \textit{CyCADA} with \textit{shift loss}, trained on single frames; we refer to this as the \textit{VR-Goggles}.
% \end{itemize}


We pretrain the segmentation network $f_{\bX}$ using \textit{Deeplab} \cite{chen2016deeplab}.
% \hl{(should say that the cycada paper actually did not use sem loss in their experiments, NEED TO DOUBLE CHECK, and they did not cos of the memory issue, we make it work by cropping, and stablize the training by cropping from the same position).}
It is worth mentioning that the original \textit{CyCADA} paper did not use the semantic constraint in their experiments due to memory issues.
We are able to incorporate semantic loss calculation, by cropping the input images\footnote{Actually, a naive random crop would highly likely lead to semantic permutations; so we crop inputs of the two domains in the same training iteration from the same random position, and our empirical results show that this greatly stabilizes the adaptation}. The input images are of size $450\times800$, we train the network with $256\times256$ crops.
We use the same network architecture as in \textit{CycleGAN},
% for the generators and discriminators,
and train for $50$ epochs with a learning rate of $2e-4$, as we observe no performance gain training for longer iterations.

In Fig. \ref{fig:carla2robotcar}, we show a comparison of the subsequent frames generated by the three approaches. Our method again achieves the highest consistency and eliminates more artifacts due to the smoothness of the learned model.


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{llcclcccccc}
\hline
                                                                                                        &                      & \multicolumn{2}{c}{training}                                                                                                                           &  & \multicolumn{6}{c}{testing}                                                               \\ \cline{3-11}
                                                                                                        &                      & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}single\\ condition\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}domain\\ random\end{tabular}} &  & \multicolumn{3}{c}{single condition} & \multicolumn{3}{c}{domain random}                  \\
                                                                                                        &                      &                                                                             &                                                                          &  & raw  & Cyc-G         & ours          & raw                & Cyc-G         & ours          \\ \hline
\multirow{4}{*}{sucess rate (\%)}                                                                       & Straight             & 81.3                                                                        & 97.3                                                                     &  & 13.3 & \textbf{93.3} & 90.7          & 64.0               & 96.0          & \textbf{100}  \\
                                                                                                        & One turn             & 64.0                                                                        & 85.3                                                                     &  & 1.3  & \textbf{54.7} & \textbf{54.7} & 36.0               & 61.3          & \textbf{76.0} \\
                                                                                                        & Navigation           & 60.0                                                                        & 84.0                                                                     &  & 0.0  & 21.3          & \textbf{45.3} & 0.0                & 42.7          & \textbf{61.3} \\
                                                                                                        & Nav. dynamic         & 58.7                                                                        & 74.7                                                                     &  & 0.0  & 21.3          & \textbf{32.0} & 0.0                & 34.7          & \textbf{56.0} \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}average percentage \\ of distance to goal (\%)\end{tabular}} & Straight             & 89.7                                                                        & 96.5                                                                     &  & 37.8 & \textbf{95.8} & 94.7          & 83.6               & 95.9          & \textbf{98.3} \\
                                                                                                        & One turn             & 73.6                                                                        & 71.1                                                                     &  & 18.4 & 36.3          & \textbf{48.4} & 24.7               & 52.0          & \textbf{71.3} \\
                                                                                                        & Navigation           & 68.6                                                                        & 88.8                                                                     &  & 7.3  & 36.7          & \textbf{51.0} & 7.4                & 60.8          & \textbf{73.1} \\
                                                                                                        & Nav. dynamic         & 68.2                                                                        & 80.7                                                                     &  & 5.0  & 32.6          & \textbf{51.3} & 5.2                & 55.7          & \textbf{72.2} \\ \hline
\multirow{5}{*}{infractions (km)}                                                                       & Opposite lane        & 2.83                                                                        & 2.55                                                                     &  & 0.23 & \textbf{0.77} & 0.72          & 0.26               & 0.83          & \textbf{2.22} \\
                                                                                                        & Sidewalk             & 6.47                                                                        & 9.70                                                                     &  & 0.21 & 1.15          & \textbf{2.62} & 0.38               & 1.29          & \textbf{2.46} \\
                                                                                                        & Collision-static     & 2.38                                                                        & 3.03                                                                     &  & 0.14 & 0.52          & \textbf{0.87} & 0.16               & 0.77          & \textbf{1.26} \\
                                                                                                        & Collision-car        & 2.06                                                                        & 1.03                                                                     &  & 0.29 & 1.01          & \textbf{1.40} & 0.27               & 0.59          & \textbf{0.77} \\
                                                                                                        & Collision-pedestrian & 15.10                                                                       & 16.17                                                                    &  & 2.17 & 4.03          & \textbf{6.98} & \textgreater{}4.60 & \textbf{7.29} & 4.67          \\ \hline
\end{tabular}
\end{table*}

% \vspace{-0.2in}

% \begin{figure}[t]
%     % \begin{tabular}{m{1in} m{0.8in} m{1in}}
%     % \centering
%     %     \includegraphics[height=0.6in]{imgs/domain_adapt/carla2robotcar/robotcar/real_B_1_0685}
%     %     &
%     %     % \begin{tabular}{m{0.5in} m{0.5in}}
%     %     \begin{tabular}{cc}
%     %         \includegraphics[height=0.3in]{imgs/domain_adapt/carla2robotcar/carla/style_001}
%     %         &
%     %         \includegraphics[height=0.3in]{imgs/domain_adapt/carla2robotcar/carla/style_002}
%     %         \\
%     %         \includegraphics[height=0.3in]{imgs/domain_adapt/carla2robotcar/carla/style_003}
%     %         &
%     %         \includegraphics[height=0.3in]{imgs/domain_adapt/carla2robotcar/carla/style_004}
%     %     \end{tabular}
%     %     &
%     %     \includegraphics[height=0.6in]{imgs/domain_adapt/carla2robotcar/robotcar/real_B_1_0686}
%     % \end{tabular}
%     %\begin{tabular}{m{0.7in} m{1.2in} m{0.7in}}
%     \begin{tabular}{m{1.1in} m{0.8in} m{1.1in}}
%     % \begin{tabular}{ccc}
%     \centering
%         \includegraphics[height=0.55in]{imgs/domain_adapt/carla2robotcar/robotcar/real_B_1_0685}
%         &
%         % % \begin{tabular}{m{0.5in} m{0.5in}}
%         % \begin{tabular}{cc}
%         %     \includegraphics[height=0.5in]{imgs/domain_adapt/carla2robotcar/carla/style_001}
%         %     &
%         %     \includegraphics[height=0.5in]{imgs/domain_adapt/carla2robotcar/carla/style_002}
%         %     \\
%         %     \includegraphics[height=0.5in]{imgs/domain_adapt/carla2robotcar/carla/style_003}
%         %     &
%         %     \includegraphics[height=0.5in]{imgs/domain_adapt/carla2robotcar/carla/style_004}
%         % \end{tabular}
%         % \includegraphics[height=0.5in]{imgs/domain_adapt/carla2robotcar/carla/style_full_000}
%         \begin{overpic}[height=0.4in]
%             {imgs/domain_adapt/carla2robotcar/carla/style_full_000}
%             \put(-10,10){\includegraphics[height=0.4in,cframe=black]{imgs/domain_adapt/carla2robotcar/carla/style_full_001}}
%             \put(10,-10){\includegraphics[height=0.4in,cframe=black]{imgs/domain_adapt/carla2robotcar/carla/style_full_003}}
%             \put(0,0){\includegraphics[height=0.4in,cframe=black]{imgs/domain_adapt/carla2robotcar/carla/style_full_000}}
%         \end{overpic}
%         &
%         \includegraphics[height=0.55in]{imgs/domain_adapt/carla2robotcar/robotcar/real_B_1_0686}
%     \end{tabular}
%     \begin{tabular}{m{1.5in} m{1.5in}}
%         \begin{overpic}[height=.9in]
%             {imgs/domain_adapt/carla2robotcar/diff/bsl_0_bbx}
%             \put(20,40){\includegraphics[height=0.2in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/bsl_0_0_big}}
%             \put(11.45,42.25){\includegraphics[height=0.1in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/bsl_0_0_small}}
%             \put(85,35){\includegraphics[height=0.2in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/bsl_0_1_big}}
%             \put(91.3,26.2){\includegraphics[height=0.1in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/bsl_0_1_small}}
%             \put(65,23){\includegraphics[height=0.2in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/bsl_0_2_big}}
%             \put(81.3,26.2){\includegraphics[height=0.1in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/bsl_0_2_small}}
%         \end{overpic}
%         &
%         \begin{overpic}[height=.9in]
%             {imgs/domain_adapt/carla2robotcar/diff/bsl_1_bbx}
%             \put(20,40){\includegraphics[height=0.2in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/bsl_1_0_big}}
%             \put(11.45,42.25){\includegraphics[height=0.1in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/bsl_1_0_small}}
%             \put(85,35){\includegraphics[height=0.2in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/bsl_1_1_big}}
%             \put(91.3,26.2){\includegraphics[height=0.1in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/bsl_1_1_small}}
%             \put(65,23){\includegraphics[height=0.2in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/bsl_1_2_big}}
%             \put(81.3,26.2){\includegraphics[height=0.1in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/bsl_1_2_small}}
%         \end{overpic}
%         \\
%         \begin{overpic}[height=.9in]
%             {imgs/domain_adapt/carla2robotcar/diff/stn_0_bbx}
%             \put(16,20){\includegraphics[height=0.2in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/stn_0_1_big}}
%             \put(31.3,22.45){\includegraphics[height=0.1in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/stn_0_1_small}}
%             % \put(46.5,20){\includegraphics[height=0.2in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/stn_0_2_big}}
%             % \put(37.55,22.45){\includegraphics[height=0.1in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/stn_0_2_small}}
%             \put(75,23){\includegraphics[height=0.2in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/stn_0_0_big}}
%             \put(90.7,26.2){\includegraphics[height=0.1in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/stn_0_0_small}}
%         \end{overpic}
%         &
%         \begin{overpic}[height=.9in]
%             {imgs/domain_adapt/carla2robotcar/diff/stn_1_bbx}
%             \put(16,20){\includegraphics[height=0.2in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/stn_1_1_big}}
%             \put(31.3,22.5){\includegraphics[height=0.1in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/stn_1_1_small}}
%             % \put(46.5,20){\includegraphics[height=0.2in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/stn_1_2_big}}
%             % \put(37.55,22.45){\includegraphics[height=0.1in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/stn_1_2_small}}
%             \put(75,23){\includegraphics[height=0.2in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/stn_1_0_big}}
%             \put(90.7,26.2){\includegraphics[height=0.1in,cframe=white]{imgs/domain_adapt/carla2robotcar/diff/stn_1_0_small}}
%         \end{overpic}
%         \\
%         \includegraphics[height=0.9in]{imgs/domain_adapt/carla2robotcar/diff/sft_0_bbx}
%         &
%         \includegraphics[height=0.9in]{imgs/domain_adapt/carla2robotcar/diff/sft_1_bbx}
%     \end{tabular}
%     \caption{
%     Comparison of the translated images for sequential input frames for different approaches.
%     $\nth{1}$ \textit{row}: two subsequent input frames from the realistic domain, with several representative images from the simulated domain shown in between;
%     $\nth{2}\sim\nth{4}$ \textit{row}: outputs from \textit{CyCADA}, \textit{CyCADA+flow} and \textit{Ours}.
%     Our method is able to output consistent subsequent frames and eliminating artifacts.
%     We adjust the brightness of some zoomins for visualization.}
%     \label{fig:carla2robotcar}
% \end{figure}


==> secs/experiments-transfer-comparison.tex <==
\subsection{Comparing Policy Transfer Methods: Simulated Indoor Navigation}
\label{sec:experiments-transfer-comparison}

\begin{figure}[!b]
    \centering
        \includegraphics[width=0.8\columnwidth]{imgs/domain_randomization}
    % \vspace{-0.1in}
    \caption{
8 different sets of textures of the 8 workers for training \textit{Multi-Domain}
%our A3C variant of \textit{Randomization}
(Sec. \ref{sec:experiments-transfer-comparison}).
    }
    \label{fig:domain-randomization}
\end{figure}

\begin{figure*}[!t]
    \hspace{0.3in}\includegraphics[width=.9\textwidth]{imgs/transfer_compare}
    \vspace{-0.1in}
    \caption{
Average episode lengths in evaluation during training,
comparing policy transfer procedures of \textit{From-Scratch}, \textit{Multi-Domain} and \textit{Progressive}.
We show median-filtered curves in line with \cite{rusu2016sim}.
An adapting phase is necessary for \textit{Progressive} in each new environment; while for our \textit{real-to-sim} approach,
\textit{From-Scratch} is all the policy training needed.
}
    \label{fig:transfer-compare}
\end{figure*}


To illustrate the difference between the policy transfer pipelines
of our proposed \textit{real-to-sim} approach
and several representative \textit{sim-to-real} approaches
%discussed in Sec. \ref{sec:related-da-drl},
we conduct a direct comparison in a simulated indoor navigation experiment.

We build an indoor office environment in \textit{Gazebo} \cite{koenig2004design}.
With two different sets of textures,
we render two environments:
\textit{\textbf{Sim-Env}} and
\textit{\textbf{"Real"-Env}}, shown on the left of Fig. \ref{fig:transfer-compare}.
We train agents to learn navigation policies
to accomplish the task of navigating to chairs based purely on its front-facing color camera readings; the agent obtained a reward of $-0.005$ for a step cost, $-0.05$ for collision, and $1$ for reaching the target.
We illustrate the procedures of the following approaches to transfer policies learned in \textit{Sim-Env} to \textit{"Real"-Env},
and show the average steps obtained by the agents in evaluation during training in Fig. \ref{fig:transfer-compare}:

(1) \textit{\textbf{From-Scratch}} \cite{mnih2016asynchronous}:
Canonical A3C trained from scratch on \textit{Sim-Env}.
We execute 8 training processes and 1 evaluation process,
each with their own copy of \textit{Sim-Env}.
We note here that this is all the policy training required for our \textit{real-to-sim} approach,
as no fine-tuning or retraining of the policy is needed for deploying it in real-world scenes;
also, since our approach decouples the policy training and the domain adaptation,
the adaptation networks can be trained in parallel with the policy training.
This is also the policy training procedure for several sim-to-real approaches
\cite{bousmalis2017using,stein2018genesis},
except that an additional adaptation step has to be added for each of the training frames;
also, for each visually different real-world scene,
this line of approaches needs to go through another complete policy training procedure.
(2) \textit{\textbf{Multi-Domain}} (inspired by \cite{Sadeghi2017cadrl, tobin2017domain}):
Our A3C variant of the \textit{domain randomization} approach.
The key concept of \textit{domain randomization} \cite{Sadeghi2017cadrl,tobin2017domain} is randomizing the textures, viewing angles, etc. of objects during the training in simulation,
such that when deploying the trained model in real-world scenarios,
the modality of the real-world objects could just be naturally dealt with as another variation.
Here we adopt the same basic idea but implement it under the constraints of our simulator
(changing the texture for each frame is not as straightforward in \textit{Gazebo}).
In detail,
each of the 8 A3C workers renders its environment with its own set of textures.
All 8 sets of textures for the various objects in the environment are shown in Fig. \ref{fig:domain-randomization}.
The evaluation during training uses \textit{Sim-Env} as its environment.
We note here that this is all the policy training required for the \textit{Multi-Domain} approach,
since once converged, the agent is expected to be directly deployable in real-world environments.
Unfortunately, for our considered task and setup,
our A3C variant of the approach does not manage to learn useful policies,
as is shown by the green dashed line in Fig. \ref{fig:transfer-compare}
(we trained it for 8 times the iterations shown but still it fails to converge).
We suspect that our variant of randomizing textures might have imposed challenges for our RL task where informative reward signals are sparse. We suspect that more workers with more sets of textures could lead to improved performance. However, with relatively limited computing resources and with simulators where there is no relatively efficient solutions for randomizing the textures of objects at each frame, the \textit{Multi-Domain} method does not learn useful policies.
%may not enough for this task.
%Considering the higher cost to design randomized environments in \textit{Gazebo},
% It shows that domain randomization may not be applicable in simulated environments like \textit{Gazebo} which costs too many efforts for texture randomization.
% We suspect that different from the supervised learning task presented by \cite{tobin2017domain}
% where the supervision signal is strong and direct,
% with the sparse and delayed reward signals in our reinforcement learning task,
% the randomization might have imposed too many challenges for learning useful policies.
(3) \textit{\textbf{Progressive}} \cite{rusu2016sim}:
\textit{Progressive Nets} for transferring the policy of \textit{From-Scratch} on \textit{Sim-Env} to \textit{"Real"-Env}.
As described in \cite{rusu2016sim},
a second column is added after the first column is trained (the \textit{From-Scratch} policy on \textit{Sim-Env}).
% \footnote{We follow the same parameter initialization strategy as in \cite{rusu2016sim} for the output layers and the connection layers
% to guarantee that the initial policy output of the agent is identical to the first column.
% Observing that the simulation and real-world environments presented in \cite{rusu2016sim} are relateively more visually similar than \textit{Sim-Env} and \textit{"Real"-Env1},
% we additionally conduct experiments where we do not incorporate the above parameter initialization strategy,
% as we suspect that a random initialization might be more beneficial for transfer scenarios where
% two environments are more visually different.
% We found out that both the identical and the random initialization works,
% with the former converging faster.
% So we only report the experiments with the identical initialization,
% shown in the blue line in Fig. \ref{fig:transfer-compare}.}.
We note that for this approach,
although the adaptation of the policy in new environments is significantly accelerated compared to training from scratch,
the overall policy training needed contains both the initial training
(the yellow block),
and an adapting phase (the cyan blocks) in case we want to deploy
the agent in new environments.%,
% e.g., \textit{Real-Env2}, \textit{Real-Env3}.


% Having illustrated the advantage of our method in the \textit{policy training} part,
% we continue to compare different approaches of implementing the \textit{domain adaptation} part for our \textit{real-to-sim} approach.

% \hl{How long time do we need to train an domain adaptation model to deploy our policy in "Real"-Env?}

% We believe the experiments and discussions above validate our setout objective
% \hl{of proposing a lightweight, flexible and efficient solution} for dealing with the \textit{reality gap}.
%
% Having illustrated the policy training part, in the next section, we compare different approaches of implementing the \textit{domain adaptation} part for our \textit{real-to-sim} approach.

